Deep Drone Racing: Learning Agile Flight in Dynamic Environments

Autonomous agile flight brings up fundamental challenges in robotics, such as coping with unreliable state estimation, reacting optimally to dynamically changing environments, and coupling perception and action in real time under severe resource constraints. In this paper, we consider these challenges in the context of autonomous, vision-based drone racing in dynamic environments. Our approach combines a convolutional neural network (CNN) with a state-of-the-art path-planning and control system. The CNN directly maps raw images into a robust representation in the form of a waypoint and desired speed. This information is then used by the planner to generate a short, minimum-jerk trajectory segment and corresponding motor commands to reach the desired goal. We demonstrate our method in autonomous agile flight scenarios, in which a vision-based quadrotor traverses drone-racing tracks with possibly moving gates. Our method does not require any explicit map of the environment and runs fully onboard. We extensively test the precision and robustness of the approach in simulation and in the physical world. We also evaluate our method against state-of-the-art navigation approaches and professional human drone pilots.

==> Makefile <==
# The target that we want to build, TODO: change name if required
targets=root.pdf

# Dependencies, all files which are taken into consideration when make decides
# if rebuilding is necessary
deps=$(wildcard */*.tex) $(wildcard images/*.png) $(wildcard images/*.jpg) \
	$(wildcard images/*.jpeg) $(wildcard images/*.pdf) \
	$(wildcard bibliography/*.bib)

# NOTE: you should note change anything below
%.pdf: %.tex $(deps) Makefile build
	# cd to build and build the report
	cd build && TEXINPUTS=../:../packages:${TEXINPUTS} pdflatex --shell-escape $<
	cd build && BIBINPUTS=../:${BIBINPUTS} BSTINPUTS=../:${BSTINPUTS} bibtex $*
	cd build && TEXINPUTS=../:../packages:${TEXINPUTS} pdflatex --shell-escape $< 
	cd build && TEXINPUTS=../:../packages:${TEXINPUTS} pdflatex --shell-escape $< 
	# copy the resulting pdf back to the main directory (mv is no good, because
	# make will rebuild even if nothing has changed)
	cp build/$@ .

all: $(targets)

clean: buildclean

build:
	# make sure that build exists
	mkdir -p build

buildclean:
	# remove the build folder
	rm -rf build *~ */*~ 

distclean: clean
	# remove the build folder (clean) and the target pdf
	rm -f $(targets)

installdeb:
	# required packages to use this makefile
	sudo apt-get install texlive texlive-math-extra

.PHONY: clean buildclean distclean all dist installdeb

